FanChuan: A Multilingual and Graph-Structured Benchmark For Parody Detection and Analysis

Parody is an emerging phenomenon on social media, where individuals imitate a role or position opposite to their own, often for humor, provocation, or controversy. Detecting and analyzing parody can be challenging and is often reliant on context, yet it plays a crucial role in understanding cultural values, promoting subcultures, and enhancing self-expression. However, the study of parody is hindered by limited available data and deficient diversity in current datasets. To bridge this gap, we built seven parody datasets from both English and Chinese corpora, with 14,755 annotated users and 21,210 annotated comments in total. To provide sufficient context information, we also collect replies and construct user-interaction graphs to provide richer contextual information, which is lacking in existing datasets. With these datasets, we test traditional methods and Large Language Models (LLMs) on three key tasks: (1) parody detection, (2) comment sentiment analysis with parody, and (3) user sentiment analysis with parody. Our extensive experiments reveal that parody-related tasks still remain challenging for all models, and contextual information plays a critical role. Interestingly, we find that, in certain scenarios, traditional sentence embedding methods combined with simple classifiers can outperform advanced LLMs, i.e. DeepSeek-R1 and GPT-o3, highlighting parody as a significant challenge for LLMs.

==> tables/context.tex <==
\begin{table*}[ht]
\centering
\caption{Parody detection with context}
\label{tab:user_senti_cls}
\resizebox{1\textwidth}{!}{
\begin{tabular}{ll|ccc|ccc|ccc|ccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Paradigm}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Alibaba-Math}} & \multicolumn{3}{c}{\textbf{BridePrice}} & \multicolumn{3}{c}{\textbf{Student-He}} & \multicolumn{3}{c}{\textbf{CS2}} & \multicolumn{3}{c}{\textbf{CampusLife}} & \multicolumn{3}{c}{\textbf{Tiktok-Trump}} & \multicolumn{3}{c}{\textbf{Reddit-Trump}} \\ \cline{3-23}
& & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R}& \textbf{F1} \\
\midrule
\multirow{3}{*}{Embedding-based} 
& BoW+MLP & 12.79 & 13.06 & 12.92 & 16.15 & 19.09 & 17.50 & 11.17 & 12.50 & 12.12 & 16.95 & 16.95 & 16.95 & 11.85 & 13.91 & 12.80 & 23.33 & 17.50 & 20.00 & 13.08 & 15.11 & 14.02 \\
& Skip-gram+MLP & 14.95 & 15.28 & 15.12 & 23.85 & 28.18 & 25.83 & 14.71 & 15.62 & 15.15 & 15.93 & 15.93 & 15.93 & 10.37 & 12.17 & 11.20 & 22.67 & 17.00 & 19.43 & 15.00 & 17.33 & 16.08 \\
& RoBERTa+MLP & 15.10 & 15.42 & 15.26 & 30.00 & 35.45 & 32.50 & 16.47 & 17.50 & 16.97 & 17.29 & 17.29 & 17.29 & 14.81 & 17.39 & 16.00 & 25.33 & 19.00 & 21.71 & 26.92 & 31.11 & 28.87 \\
\midrule
\multirow{4}{*}{Inconsistency-based} 
& BNS-Net & 8.27 & 5.05 & 6.27 & 4.17 & 6.67 & 5.13 & 10.00 & 7.14 & 8.33 & 10.91 & 10.53 & 10.71 & 10.64 & 12.50 & 11.49 & 19.61 & 19.05 & 19.32 & 16.92 & 24.44 & 20.00 \\
& DC-Net & 20.00 & 10.14 & 13.46 & 33.33 & 16.67 & 22.22 & 35.00 & 17.95 & 23.73 & 14.71 & 18.52 & 16.39 & 13.64 & 25.00 & 17.65 & 14.29 & 10.00 & 11.76 & 14.41 & 30.77 & 19.63 \\
& QUIET & 11.42 & 20.44 & 14.63 & 12.01 & 21.60 & 15.41 & 3.52 & 19.64 & 5.95 & 4.72 & 11.97 & 6.76 & 9.82 & 19.87 & 13.10 & 9.46 & 24.11 & 13.56 & 13.02 & 16.50 & 14.52 \\
& SarcPrompt & 5.88 & 4.55 & 5.13 & 45.45 & 33.33 & 38.46 & 57.14 & 9.52 & 16.33 & 11.54 & 20.34 & 14.72 & 16.67 & 13.04 & 14.63 & 23.53 & 30.00 & 26.37 & 24.32 & 20.00 & 21.95 \\
\midrule
\multirow{3}{*}{Unsupervised} 
& Isolation Forest & 5.73 & 5.73 & 5.73 & 1.18 & 1.19 & 1.18 & 4.39 & 4.42 & 4.41 & 8.67 & 8.67 & 8.67 & 6.74 & 6.74 & 6.74 & 8.16 & 8.25 & 8.21 & 11.11 & 11.11 & 11.11 \\
& RoBERTa+Z-Score & 12.93 & 13.76 & 13.33 & 30.77 & 36.36 & 33.33 & 5.88 & 4.76 & 5.26 & 12.70 & 14.04 & 13.33 & 23.08 & 22.50 & 22.78 & 36.36 & 34.29 & 35.29 & 30.77 & 35.56 & 32.99 \\
& One-Class SVM & 5.75 & 5.73 & 5.74 & 3.70 & 3.57 & 3.64 & 5.88 & 6.19 & 6.03 & 6.53 & 6.63 & 6.58 & 9.68 & 10.11 & 9.89 & 8.16 & 8.25 & 8.21 & 15.25 & 15.79 & 15.52 \\
\midrule
\multirow{5}{*}{LLMs} 
& ChatGPT4o & 12.49 & 44.88 & 19.54 & 10.19 & 63.10 & 17.55 & 9.30 & 53.10 & 15.83 & 15.75 & 73.47 & 25.95 & 34.33 & 51.69 & 41.26 & 22.95 & 69.07 & 34.45 & 36.76 & 58.48 & 45.15 \\
& ChatGPT4o-mini & 8.20 & 62.78 & 14.51 & 7.63 & 64.29 & 13.64 & 5.71 & 56.64 & 10.37 & 10.23 & 69.39 & 17.84 & 28.78 & 66.29 & 40.14 & 21.45 & 63.92 & 32.12 & 33.61 & 47.37 & 39.32 \\
& Claude3.5 & 7.42 & 65.90 & 13.34 & 10.62 & 60.00 & 18.05 & 8.73 & 20.37 & 12.22 & 10.42 & 58.68 & 17.71 & 25.26 & 53.93 & 34.41 & 15.31 & 63.92 & 24.70 & 32.54 & 56.14 & 41.20 \\
& Qwen2.5 & 7.69 & 85.28 & 14.11 & 7.98 & 76.19 & 14.45 & 4.94 & 61.06 & 9.15 & 9.40 & 87.76 & 16.98 & 13.95 & 94.38 & 24.31 & 10.41 & 90.72 & 18.68 & 17.00 & 90.64 & 28.62 \\
& DeepSeek-V3 & 11.08 & 56.44 & 18.52 & 6.44 & 94.05 & 12.06 & 8.98 & 38.94 & 14.59 & 15.61 & 67.86 & 25.38 & 25.29 & 73.03 & 37.57 & 13.46 & 85.26 & 23.24 & 34.16 & 56.14 & 42.48 \\
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/fanchuan.tex <==
\begin{table*}[ht]
\centering
\caption{ORP Detection}
\label{tab:ORP_detection}
\resizebox{1\textwidth}{!}{
\begin{tabular}{ll|ccc|ccc|ccc|ccc|ccc|ccc|ccc|c}
\toprule
\multirow{2}{*}{\textbf{Paradigm}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Alibaba-Math}} & \multicolumn{3}{c}{\textbf{BridePrice}} & \multicolumn{3}{c}{\textbf{Student-He}} & \multicolumn{3}{c}{\textbf{CS2}} & \multicolumn{3}{c}{\textbf{CampusLife}} & \multicolumn{3}{c}{\textbf{Tiktok-Trump}} & \multicolumn{3}{c|}{\textbf{Reddit-Trump}} & \multirow{2}{*}{\textbf{\shortstack{Ave. \\ Rank}}} \\ \cline{3-23}
& & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R}& \textbf{F1} \\
\midrule
\multirow{3}{*}{Embedding-based} 
& BoW+MLP & 10.07 & 10.28 & 10.17 & 14.62 & 17.27 & 15.83 & 8.77 & 9.38 & 9.06 & 15.93 & 15.93 & 15.93 & 10.37 & 12.17 & 11.20 & 16.00 & 12.00 & 13.71 & 15.77 & 18.22 & 16.91 & 10.29 \\
& Skip-gram+MLP & 14.01 & 14.31 & 14.16 & 16.15 & 19.09 & 17.50 & 14.12 & 15.00 & 14.55 & 17.29 & 17.29 & 17.29 & 9.63 & 11.30 & 10.40 & 18.00 & 13.50 & 15.43 & 13.85 & 16.00 & 14.85 & 8.43 \\
& RoBERTa+MLP & 14.15 & 14.44 & 14.30 & 17.69 & 20.91 & 19.17 & 12.94 & 13.75 & 13.33 & 16.61 & 16.61 & 16.61 & 19.26 & 14.07 & 16.52 & 14.00 & 10.50 & 12.00 & 21.54 & 24.89 & 23.09 & 7.29 \\
\midrule
\multirow{4}{*}{Inconsistency-based} 
& BNS-Net & 11.55 & 16.59 & 13.62 & 12.12 & 12.50 & 12.31 & 28.57 & 11.76 & \underline{16.67} & 28.12 & 15.52 & 20.00 & 28.57 & 27.78 & 28.17 & 24.21 & 25.56 & 24.86 & 18.18 & 15.38 & 16.67 & 6.86 \\
& DC-Net & 9.84 & 21.74 & 13.54 & 9.09 & 12.50 & 10.53 & 15.09 & 20.51 & \textbf{17.39} & 8.65 & 42.59 & 14.37 & 12.12 & 16.67 & 14.04 & 7.50 & 12.50 & 9.38 & 18.56 & 34.62 & 24.16 & 10.14 \\
& QUIET & 12.45 & 22.37 & \underline{15.98} & 6.75 & 23.79 & 10.75 & 2.91 & 16.40 & 4.94 & 5.42 & 13.66 & 7.75 & 9.82 & 19.70 & 13.07 & 7.03 & 18.12 & 10.11 & 14.60 & 18.62 & 16.34 & 11.43 \\
& SarcPrompt & 48.00 & 8.33 & 14.20 & 21.74 & 22.73 & \textbf{22.22} & 16.67 & 3.12 & 5.26 & 15.62 & 33.90 & \textbf{21.39} & 57.14 & 17.39 & 26.67 & 11.11 & 25.00 & 15.38 & 13.11 & 17.78 & 15.09 & 7.29 \\
\midrule
\multirow{3}{*}{Outlier Detection} 
& Isolation Forest & 5.93 & 5.93 & 5.93 & 1.18 & 1.19 & 1.18 & 0.91 & 0.88 & 0.90 & 7.14 & 7.14 & 7.14 & 5.62 & 5.62 & 5.62 & 6.12 & 6.19 & 6.15 & 11.70 & 11.70 & 11.70 & 15.71 \\
& RoBERTa+Z-Score & 12.93 & 13.19 & 13.06 & 19.23 & 22.73 & \underline{20.83} & 12.12 & 12.50 & 12.31 & 18.64 & 18.64 & 18.64 & 18.18 & 17.39 & 17.78 & 16.67 & 12.50 & 14.29 & 32.00 & 17.78 & 22.68 & 7.71 \\
& One-Class SVM & 5.89 & 5.73 & 5.81 & 4.65 & 4.76 & 4.71 & 1.82 & 1.77 & 1.79 & 5.67 & 5.61 & 5.64 & 7.78 & 7.87 & 7.82 & 9.00 & 9.28 & 9.14 & 14.77 & 15.20 & 14.99 & 15.14 \\
\midrule
\multirow{7}{*}{LLMs} 
& ChatGPT4o & 9.09 & 63.58 & 15.90 & 7.48 & 71.43 & 13.54 & 4.96 & 45.45 & 8.94 & 10.95 & 68.04 & 18.86 & 34.89 & 33.71 & 34.29 & 32.88 & 49.48 & \textbf{39.51} & 25.28 & 70.83 & \textbf{37.26} & \textbf{3.86} \\
& ChatGPT4o-mini & 7.82 & 55.83 & 13.73 & 6.07 & 61.90 & 11.06 & 4.97 & 42.48 & 8.91 & 9.52 & 50.00 & 16.00 & 31.06 & 56.18 & \underline{40.00} & 24.47 & 71.13 & \underline{36.41} & 25.69 & 65.50 & \underline{36.90} & 6.64 \\
& Claude3.5 & 7.25 & 74.69 & 13.21 & 6.74 & 85.71 & 12.49 & 4.64 & 55.45 & 8.56 & 9.00 & 58.25 & 16.00 & 29.70 & 67.42 & \textbf{41.24} & 19.05 & 70.10 & 29.96 & 24.69 & 69.59 & 36.45 & 6.93 \\
& Qwen2.5 & 8.48 & 60.33 & 14.88 & 6.86 & 66.67 & 12.44 & 4.31 & 41.59 & 7.81 & 11.48 & 62.24 & 19.38 & 18.01 & 73.03 & 28.89 & 16.78 & 79.38 & 27.70 & 21.40 & 74.85 & 33.29 & 6.29 \\
& DeepSeek-V3 & 9.34 & 59.92 & \textbf{16.17} & 7.31 & 70.24 & 13.24 & 5.18 & 40.71 & 9.19 & 12.56 & 55.10 & \underline{20.45} & 21.23 & 69.66 & 32.55 & 19.22 & 81.44 & 31.10 & 22.44 & 73.10 & 34.34 & \underline{4.86} \\
& DeepSeek-R1 & 7.90 & 76.89 & 14.33 & 6.61 & 85.71 & 12.27 & 4.29 & 60.18 & 8.01 & 9.07 & 75.00 & 16.18 & 13.11 & 84.27 & 22.69 & 11.93 & 88.66 & 21.03 & 18.54 & 81.87 & 30.24 & 8.14 \\
& ChatGPT-o3-mini & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
& ChatGPT-o1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
\bottomrule
\end{tabular}
}
\end{table*}



\begin{table*}[ht]
\centering
\caption{New Template (Delete this after finishing)}
\label{tab:ORP_detection}
\resizebox{1\textwidth}{!}{
\begin{tabular}{ll|ccccccc|c}
\toprule
\textbf{Paradigm} & \textbf{Method} & \textbf{Alibaba.} & \textbf{Bride.} & \textbf{Student.} & \textbf{CS2} & \textbf{Campus.} & \textbf{Tiktok.} & \textbf{Reddit.} & \textbf{Ave. Rank} \\
\midrule
\multirow{3}{*}{Embedding-based} 
& BoW+MLP & 10.07 & 10.28 & 10.17 & 14.62 & 17.27 & 15.83 & 8.77 & 9.38  \\
& Skip-gram+MLP & 10.07 & 10.28 & 10.17 & 14.62 & 17.27 & 15.83 & 8.77 & 9.38  \\
& RoBERTa+MLP & 10.07 & 10.28 & 10.17 & 14.62 & 17.27 & 15.83 & 8.77 & 9.38  \\
\bottomrule
\end{tabular}
}
\end{table*}




==> tables/sentiment.tex <==
\begin{table*}[ht]
\centering
\caption{Comment sentiment classifiation.}
\label{tab:comment_senti_cls}
\resizebox{1\textwidth}{!}{
\begin{tabular}{ll|cc|cc|cc|cc|cc|cc|cc|c}
\toprule
\multirow{2}{*}{\textbf{Paradigm}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Alibaba-Math}} & \multicolumn{2}{c}{\textbf{BridePrice}} & \multicolumn{2}{c}{\textbf{Student-He}} & \multicolumn{2}{c}{\textbf{CS2}} & \multicolumn{2}{c}{\textbf{CampusLife}} & \multicolumn{2}{c}{\textbf{Tiktok-Trump}} & \multicolumn{2}{c|}{\textbf{Reddit-Trump}} & \multirow{2}{*}{\textbf{\shortstack{Ave. \\ Rank}}} \\ \cline{3-16}
& & \textbf{Macro-F1} & \textbf{Micro-F1} & \textbf{Macro-F1} & \textbf{Micro-F1} & \textbf{Macro-F1} & \textbf{Micro-F1} & \textbf{Macro-F1} & \textbf{Micro-F1} & \textbf{Macro-F1} & \textbf{Micro-F1} & \textbf{Macro-F1} & \textbf{Micro-F1} & \textbf{Macro-F1} & \textbf{Micro-F1} \\
\midrule
\multirow{3}{*}{Embedding-based} 
& BoW+MLP & 35.30 & 48.79 & \textbf{40.43} & 64.66 & \underline{48.78} & 62.81 & 27.56 & 48.45 & 32.35 & 59.45 & 33.74 & 47.27 & 37.13 & 43.41 & 6.64 \\
& Skip-gram+MLP & 39.62 & 43.26 & \underline{39.50} & 64.47 & 47.46 & 67.78 & 31.09 & 46.01 & 30.80 & 53.20 & 35.42 & 45.06 & 37.71 & 41.54 & 6.93 \\
& RoBERTa+MLP & 36.91 & 41.28 & 34.48 & 53.31 & 44.17 & 59.87 & 26.02 & 41.61 & \underline{38.87} & 63.59 & 47.56 & 60.29 & 51.66 & 58.85 & 6.07 \\
\midrule
\multirow{4}{*}{Inconsistency-based} 
& BNS-Net & 35.48 & \textbf{69.78} & 29.40 & \textbf{76.36} & 45.66 & \textbf{78.87} & 21.13 & \textbf{60.38} & 29.71 & \textbf{80.39} & 26.47 & \underline{60.90} & 22.08 & 49.40 & 5.82 \\
& DC-Net & 16.07 & 18.28 & 28.87 & \textbf{76.36} & 48.66 & \underline{75.62} & 18.89 & 58.08 & \textbf{38.90} & \underline{77.35} & 45.21 & 59.47 & 37.18 & 45.56 & 6.25 \\
& QUIET & 24.34 & 30.54 & 30.26 & 67.34 & 35.52 & 64.85 & 17.65 & 40.12 & 30.05 & 73.81 & 29.51 & 57.84 & 23.95 & 45.61 & 8.64 \\
& SarcPrompt & 28.77 & \underline{56.26} & 28.85 & 75.56 & 33.91 & 68.94 & 19.18 & 40.38 & 35.21 & 67.40 & 40.06 & 44.08 & 22.69 & 48.08 & 7.79 \\
\midrule
\multirow{5}{*}{LLMs} 
& ChatGPT4o & 40.00 & 43.69 & 32.28 & 43.26 & 47.75 & 59.26 & \textbf{37.82} & 55.91 & 32.10 & 44.19 & 51.02 & 53.31 & 51.89 & \textbf{62.36} & \underline{5.43} \\
& ChatGPT4o-mini & \underline{40.01} & 45.49 & 34.27 & 47.97 & \textbf{49.95} & 65.08 & 34.33 & 57.20 & 33.19 & 45.14 & \underline{51.56} & 53.65 & \underline{52.42} & 61.86 & \textbf{4.21} \\
& Claude3.5 & \textbf{40.53} & 44.00 & 29.89 & 37.95 & 42.99 & 57.30 & 30.70 & 46.45 & 28.31 & 36.81 & 46.03 & 48.86 & 51.92 & 60.20 & 7.50 \\
& Qwen2.5 & 38.46 & 41.88 & 31.83 & 44.14 & 46.14 & 56.87 & \underline{34.78} & 58.51 & 28.38 & 36.76 & 47.55 & 50.18 & 51.93 & 60.09 & 6.71 \\
& DeepSeek-V3 & 35.88 & 37.28 & 28.15 & 34.44 & 43.05 & 49.68 & 32.62 & \underline{58.89} & 36.36 & 54.56 & \textbf{56.26} & \textbf{62.83} & \textbf{54.83} & \underline{61.90} & 5.93 \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/sentiment_user.tex <==
\begin{table*}[ht]
\label{tab:user_senti_cls}
\centering
\caption{User sentiment classification.}
\resizebox{1\textwidth}{!}{
\begin{tabular}{ll|cc|cc|cc|cc|cc|cc|cc|c}
\toprule
\multirow{2}{*}{\textbf{Paradigm}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Alibaba-Math}} & \multicolumn{2}{c}{\textbf{BridePrice}} & \multicolumn{2}{c}{\textbf{Student-He}} & \multicolumn{2}{c}{\textbf{CS2}} & \multicolumn{2}{c}{\textbf{CampusLife}} & \multicolumn{2}{c}{\textbf{Tiktok-Trump}} & \multicolumn{2}{c|}{\textbf{Reddit-Trump}} & \multirow{2}{*}{\textbf{\shortstack{Ave. \\ Rank}}} \\ \cline{3-16}
& & \textbf{Macro-F1} & \textbf{Micro-F1} & \textbf{Macro-F1} & \textbf{Micro-F1} & \textbf{Macro-F1} & \textbf{Micro-F1} & \textbf{Macro-F1} & \textbf{Micro-F1} & \textbf{Macro-F1} & \textbf{Micro-F1} & \textbf{Macro-F1} & \textbf{Micro-F1} & \textbf{Macro-F1} & \textbf{Micro-F1} \\
\midrule
\multirow{3}{*}{Embedding-based} 
& BoW+MLP & \underline{46.54} & 48.74 & 37.60 & 60.90 & 46.65 & 60.41 & 29.22 & 43.03 & 32.35 & 52.16 & 35.05 & 44.53 & 31.97 & 40.17 & 0 \\
& Skip-gram+MLP & \textbf{46.99} & 48.75 & 38.28 & 59.26 & 50.45 & 64.54 & 31.92 & 45.38 & 32.02 & 52.63 & 38.46 & 47.28 & 32.69 & 42.49 & 0 \\
& RoBERTa+MLP & 43.11 & 45.77 & 36.94 & 61.01 & 44.20 & 63.12 & 27.09 & 42.90 & 35.49 & 61.64 & 50.82 & 60.22 & 52.79 & 58.32 & 0 \\
\midrule
\multirow{3}{*}{Inconsistency-based} 
& BNS-Net & 34.32 & 49.38 & 27.21 & 68.97 & 41.91 & 78.33 & 23.38 & 60.19 & 28.67 & 75.44 & 23.61 & 54.84 & 22.98 & 52.60 & 0 \\
& DC-Net & 16.51 & 26.92 & 33.56 & 63.13 & 48.65 & 68.30 & 17.17 & 42.36 & 35.60 & 75.44 & 34.62 & 49.73 & 39.54 & 50.29 & 0 \\
& SarcPrompt & 27.72 & 53.75 & 38.54 & 71.81 & 29.51 & 79.40 & 15.62 & 57.80 & 31.45 & 69.01 & 24.48 & 53.37 & 39.10 & 56.52 & 0 \\
\midrule
\multirow{3}{*}{Graph-based} 
& GCN & 23.07 & \textbf{52.92} & 39.45 & 69.95 & 44.70 & 72.22 & 14.65 & 57.80 & 36.18 & 65.50 & 30.48 & 56.33 & 48.09 & 58.26 & 0 \\
& GAT & 23.29 & 52.67 & 37.63 & 65.69 & 45.22 & 76.80 & 15.65 & 57.96 & 37.64 & 65.50 & 43.19 & 54.99 & 48.63 & 57.10 & 0 \\
& GraphSAGE & 23.07 & \textbf{52.92} & 37.78 & 69.68 & 45.22 & 75.03 & 14.65 & 57.80 & 32.37 & 63.16 & 41.12 & 56.87 & 51.31 & 60.00 & 0 \\
\midrule
\multirow{5}{*}{LLMs} 
& ChatGPT4o & 41.71 & 44.62 & 35.02 & 46.73 & 51.54 & 65.18 & 39.19 & 56.52 & 35.89 & 45.87 & 45.87 & 51.50 & 49.01 & 60.82 & 0 \\
& ChatGPT4o-mini & 40.55 & 41.47 & 30.25 & 37.88 & 45.88 & 54.95 & 34.03 & 49.59 & 31.95 & 39.57 & 45.29 & 49.39 & 51.20 & 61.30 & 0 \\
& Claude3.5 & 41.47 & 43.02 & 29.96 & 36.58 & 43.78 & 54.38 & 32.81 & 50.17 & 31.07 & 37.83 & 41.85 & 48.40 & 46.92 & 60.56 & 0 \\
& Qwen2.5 & 40.89 & 44.13 & 33.08 & 44.82 & 49.52 & 59.93 & 36.51 & 56.38 & 33.34 & 41.55 & 46.18 & 51.17 & 50.13 & 61.50 & 0 \\
& DeepSeek-V3 & 40.00 & 40.42 & 26.37 & 31.42 & 41.55 & 45.07 & 33.61 & 54.13 & 40.49 & 51.61 & 54.04 & 58.69 & 53.22 & 63.58 & 0 \\
\bottomrule
\end{tabular}
}
\end{table*}
